A Physics-based Scaling of the Charging Rate in Latent Heat Thermal Energy Storage Devices

Thermal energy storage (TES) is increasingly recognized as an essential component of efficient Combined Heat and Power (CHP), Concentrated Solar Power (CSP), Heating Ventilation and Air Conditioning (HVAC), and refrigeration as it reduces peak demand while helping to manage intermittent availability of energy (e.g., from solar or wind). Latent Heat Thermal Energy Storage (LHTES) is a viable option because of its high energy storage density. Parametric analysis of LHTES heat exchangers have been focused on obtaining data with laminar flow in the phase changing fluid and then fitting a functional form, such as a power law or polynomial, to those data. Alternatively, in this paper we present a parametric framework to analyze LHTES devices by identifying all relevant fluid parameters and corresponding dimensionless numbers. We present 64 simulations of an LHTES device using the finite volume method at four values of the Grashof, Prandtl and Reynolds numbers in the phase change material (PCM) and heat transfer fluid (HTF). We observe that with sufficient energy available in the HTF, the effects of the HTF Reynolds number and Prandtl number on the heat transfer rate are negligible. Under these conditions, we propose a time scale for the variation of energy stored (or melt fraction) of the LHTES device based on the Fourier number($Fo$), Grashof number($Gr_p$) and Prandtl number($Pr_p$) and observe a $Gr_p^1$ and $Pr_p^{(1/3)}$ dependency. We also identify two distinct regions in the variation of the melt fraction with time, namely, the linear and the asymptotic region. We also predict the critical value of the melt fraction at the transition between the two regions. From these analyses, we draw some conclusions regarding the design procedure for LHTES devices.

==> Figures/Actual_Grp-4_values_at_Ref2Prf2Prp4.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5040.00,3528.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(946,704){\makebox(0,0)[r]{\strut{}$-1.5$}}%
      \put(946,1076){\makebox(0,0)[r]{\strut{}$-1.0$}}%
      \put(946,1448){\makebox(0,0)[r]{\strut{}$-0.5$}}%
      \put(946,1820){\makebox(0,0)[r]{\strut{}$0.0$}}%
      \put(946,2191){\makebox(0,0)[r]{\strut{}$0.5$}}%
      \put(946,2563){\makebox(0,0)[r]{\strut{}$1.0$}}%
      \put(946,2935){\makebox(0,0)[r]{\strut{}$1.5$}}%
      \put(946,3307){\makebox(0,0)[r]{\strut{}$2.0$}}%
      \put(1078,484){\makebox(0,0){\strut{}$0.0$}}%
      \put(1587,484){\makebox(0,0){\strut{}$2.0$}}%
      \put(2097,484){\makebox(0,0){\strut{}$4.0$}}%
      \put(2606,484){\makebox(0,0){\strut{}$6.0$}}%
      \put(3115,484){\makebox(0,0){\strut{}$8.0$}}%
      \put(3624,484){\makebox(0,0){\strut{}$10.0$}}%
      \put(4134,484){\makebox(0,0){\strut{}$12.0$}}%
      \put(4643,484){\makebox(0,0){\strut{}$14.0$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(209,2005){\rotatebox{-270}{\makebox(0,0){\strut{}Measured $Gr_p (\times100000)$}}}%
      \put(2860,154){\makebox(0,0){\strut{}$Fo_p$}}%
      \csname LTb\endcsname%%
      \put(3656,1537){\makebox(0,0)[r]{\strut{}$Gr_p=24906$}}%
      \csname LTb\endcsname%%
      \put(3656,1317){\makebox(0,0)[r]{\strut{}$\ \ \ \  83021$}}%
      \csname LTb\endcsname%%
      \put(3656,1097){\makebox(0,0)[r]{\strut{}$\ \ \ \  141134$}}%
      \csname LTb\endcsname%%
      \put(3656,877){\makebox(0,0)[r]{\strut{}$\ \ \ \  199248$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{Actual_Grp-4_values_at_Ref2Prf2Prp4}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figures/Grp-4_values_and_Prp-4_values_at_Ref2Prf2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(9360.00,6840.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(814,704){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(814,1887){\makebox(0,0)[r]{\strut{}$0.2$}}%
      \put(814,3070){\makebox(0,0)[r]{\strut{}$0.4$}}%
      \put(814,4253){\makebox(0,0)[r]{\strut{}$0.6$}}%
      \put(814,5436){\makebox(0,0)[r]{\strut{}$0.8$}}%
      \put(814,6619){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(946,484){\makebox(0,0){\strut{}$0.0$}}%
      \put(2549,484){\makebox(0,0){\strut{}$2.0$}}%
      \put(4153,484){\makebox(0,0){\strut{}$4.0$}}%
      \put(5756,484){\makebox(0,0){\strut{}$6.0$}}%
      \put(7360,484){\makebox(0,0){\strut{}$8.0$}}%
      \put(8963,484){\makebox(0,0){\strut{}$10.0$}}%
      \put(1748,6323){\makebox(0,0)[l]{\strut{}$\eta_{crtical}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(209,3661){\rotatebox{-270}{\makebox(0,0){\strut{}$\eta_{\tau}(\tau)$}}}%
      \put(4954,154){\makebox(0,0){\strut{}$\tau |_{Re_f2,Pr_f2} = Pr_p^{1/3} Gr_p Fo_p (\times100000)$}}%
      \csname LTb\endcsname%%
      \put(7976,5311){\makebox(0,0)[r]{\strut{}$Gr_p=24906\ Pr_p=57$}}%
      \csname LTb\endcsname%%
      \put(7976,5091){\makebox(0,0)[r]{\strut{}$83021\ \ \ \ \ \ \ \ \ \ 57$}}%
      \csname LTb\endcsname%%
      \put(7976,4871){\makebox(0,0)[r]{\strut{}$141134\ \ \ \ \ \ \ \ \ \ 57$}}%
      \csname LTb\endcsname%%
      \put(7976,4651){\makebox(0,0)[r]{\strut{}$199248\ \ \ \ \ \ \ \ \ \ 57$}}%
      \csname LTb\endcsname%%
      \put(7976,4431){\makebox(0,0)[r]{\strut{}$24906\ \ \ \ \ \ \ \ \ \ 14$}}%
      \csname LTb\endcsname%%
      \put(7976,4211){\makebox(0,0)[r]{\strut{}$83021\ \ \ \ \ \ \ \ \ \ 14$}}%
      \csname LTb\endcsname%%
      \put(7976,3991){\makebox(0,0)[r]{\strut{}$141134\ \ \ \ \ \ \ \ \ \ 14$}}%
      \csname LTb\endcsname%%
      \put(7976,3771){\makebox(0,0)[r]{\strut{}$199248\ \ \ \ \ \ \ \ \ \ 14$}}%
      \csname LTb\endcsname%%
      \put(7976,3551){\makebox(0,0)[r]{\strut{}$24906\ \ \ \ \ \ \ \ \ \ 8$}}%
      \csname LTb\endcsname%%
      \put(7976,3331){\makebox(0,0)[r]{\strut{}$83021\ \ \ \ \ \ \ \ \ \ 8$}}%
      \csname LTb\endcsname%%
      \put(7976,3111){\makebox(0,0)[r]{\strut{}$141134\ \ \ \ \ \ \ \ \ \ 8$}}%
      \csname LTb\endcsname%%
      \put(7976,2891){\makebox(0,0)[r]{\strut{}$199248\ \ \ \ \ \ \ \ \ \ 8$}}%
      \csname LTb\endcsname%%
      \put(7976,2671){\makebox(0,0)[r]{\strut{}$24906\ \ \ \ \ \ \ \ \ \ 6$}}%
      \csname LTb\endcsname%%
      \put(7976,2451){\makebox(0,0)[r]{\strut{}$83021\ \ \ \ \ \ \ \ \ \ 6$}}%
      \csname LTb\endcsname%%
      \put(7976,2231){\makebox(0,0)[r]{\strut{}$141134\ \ \ \ \ \ \ \ \ \ 6$}}%
      \csname LTb\endcsname%%
      \put(7976,2011){\makebox(0,0)[r]{\strut{}$199248\ \ \ \ \ \ \ \ \ \ 6$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{Grp-4_values_and_Prp-4_values_at_Ref2Prf2}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figures/Grp-4_values_at_Ref2Prf2Prp2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5040.00,3528.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(814,704){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(814,1225){\makebox(0,0)[r]{\strut{}$0.2$}}%
      \put(814,1745){\makebox(0,0)[r]{\strut{}$0.4$}}%
      \put(814,2266){\makebox(0,0)[r]{\strut{}$0.6$}}%
      \put(814,2786){\makebox(0,0)[r]{\strut{}$0.8$}}%
      \put(814,3307){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(946,484){\makebox(0,0){\strut{}$0.0$}}%
      \put(1685,484){\makebox(0,0){\strut{}$1.0$}}%
      \put(2425,484){\makebox(0,0){\strut{}$2.0$}}%
      \put(3164,484){\makebox(0,0){\strut{}$3.0$}}%
      \put(3904,484){\makebox(0,0){\strut{}$4.0$}}%
      \put(4643,484){\makebox(0,0){\strut{}$5.0$}}%
      \put(1316,3177){\makebox(0,0)[l]{\strut{}$\eta_{crtical}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(209,2005){\rotatebox{-270}{\makebox(0,0){\strut{}$\eta_\tau$}}}%
      \put(2794,154){\makebox(0,0){\strut{}$\taupg = Gr_p Fo_p (\times100000)$}}%
      \csname LTb\endcsname%%
      \put(3656,2335){\makebox(0,0)[r]{\strut{}$Gr_p = 24906$}}%
      \csname LTb\endcsname%%
      \put(3656,2115){\makebox(0,0)[r]{\strut{}$\ \ \ \   83021$}}%
      \csname LTb\endcsname%%
      \put(3656,1895){\makebox(0,0)[r]{\strut{}$\ \ \ \   141134$}}%
      \csname LTb\endcsname%%
      \put(3656,1675){\makebox(0,0)[r]{\strut{}$\ \ \ \   199248$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{Grp-4_values_at_Ref2Prf2Prp2}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figures/Grp-4_values_at_Ref2Prf2Prp4.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5040.00,3528.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(814,704){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(814,1225){\makebox(0,0)[r]{\strut{}$0.2$}}%
      \put(814,1745){\makebox(0,0)[r]{\strut{}$0.4$}}%
      \put(814,2266){\makebox(0,0)[r]{\strut{}$0.6$}}%
      \put(814,2786){\makebox(0,0)[r]{\strut{}$0.8$}}%
      \put(814,3307){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(946,484){\makebox(0,0){\strut{}$0.0$}}%
      \put(1685,484){\makebox(0,0){\strut{}$1.0$}}%
      \put(2425,484){\makebox(0,0){\strut{}$2.0$}}%
      \put(3164,484){\makebox(0,0){\strut{}$3.0$}}%
      \put(3904,484){\makebox(0,0){\strut{}$4.0$}}%
      \put(4643,484){\makebox(0,0){\strut{}$5.0$}}%
      \put(1316,3177){\makebox(0,0)[l]{\strut{}$\eta_{crtical}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(209,2005){\rotatebox{-270}{\makebox(0,0){\strut{}$\eta_\tau$}}}%
      \put(2794,154){\makebox(0,0){\strut{}$\taupg = Gr_p Fo_p (\times100000)$}}%
      \csname LTb\endcsname%%
      \put(3656,2335){\makebox(0,0)[r]{\strut{}$Gr_p = 24906$}}%
      \csname LTb\endcsname%%
      \put(3656,2115){\makebox(0,0)[r]{\strut{}$\ \ \ \   83021$}}%
      \csname LTb\endcsname%%
      \put(3656,1895){\makebox(0,0)[r]{\strut{}$\ \ \ \   141134$}}%
      \csname LTb\endcsname%%
      \put(3656,1675){\makebox(0,0)[r]{\strut{}$\ \ \ \   199248$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{Grp-4_values_at_Ref2Prf2Prp4}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figures/Prf-4_values_at_Ref2Prp1Grp2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5040.00,3528.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(814,704){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(814,964){\makebox(0,0)[r]{\strut{}$0.1$}}%
      \put(814,1225){\makebox(0,0)[r]{\strut{}$0.2$}}%
      \put(814,1485){\makebox(0,0)[r]{\strut{}$0.3$}}%
      \put(814,1745){\makebox(0,0)[r]{\strut{}$0.4$}}%
      \put(814,2006){\makebox(0,0)[r]{\strut{}$0.5$}}%
      \put(814,2266){\makebox(0,0)[r]{\strut{}$0.6$}}%
      \put(814,2526){\makebox(0,0)[r]{\strut{}$0.7$}}%
      \put(814,2786){\makebox(0,0)[r]{\strut{}$0.8$}}%
      \put(814,3047){\makebox(0,0)[r]{\strut{}$0.9$}}%
      \put(814,3307){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(946,484){\makebox(0,0){\strut{}$0.0$}}%
      \put(1474,484){\makebox(0,0){\strut{}$0.2$}}%
      \put(2002,484){\makebox(0,0){\strut{}$0.4$}}%
      \put(2530,484){\makebox(0,0){\strut{}$0.6$}}%
      \put(3059,484){\makebox(0,0){\strut{}$0.8$}}%
      \put(3587,484){\makebox(0,0){\strut{}$1.0$}}%
      \put(4115,484){\makebox(0,0){\strut{}$1.2$}}%
      \put(4643,484){\makebox(0,0){\strut{}$1.4$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(209,2005){\rotatebox{-270}{\makebox(0,0){\strut{}$\eta_\tau$}}}%
      \put(2794,154){\makebox(0,0){\strut{}$\taufp = Fo_p $}}%
      \csname LTb\endcsname%%
      \put(3656,1537){\makebox(0,0)[r]{\strut{}$Pr_f = 10$}}%
      \csname LTb\endcsname%%
      \put(3656,1317){\makebox(0,0)[r]{\strut{}$\ \ \ \  8$}}%
      \csname LTb\endcsname%%
      \put(3656,1097){\makebox(0,0)[r]{\strut{}$\ \ \ \  6$}}%
      \csname LTb\endcsname%%
      \put(3656,877){\makebox(0,0)[r]{\strut{}$\ \ \ \  5$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{Prf-4_values_at_Ref2Prp1Grp2}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figures/Prp-4_values_at_Ref2Prf2Grp4.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5040.00,3528.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(814,704){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(814,964){\makebox(0,0)[r]{\strut{}$0.1$}}%
      \put(814,1225){\makebox(0,0)[r]{\strut{}$0.2$}}%
      \put(814,1485){\makebox(0,0)[r]{\strut{}$0.3$}}%
      \put(814,1745){\makebox(0,0)[r]{\strut{}$0.4$}}%
      \put(814,2006){\makebox(0,0)[r]{\strut{}$0.5$}}%
      \put(814,2266){\makebox(0,0)[r]{\strut{}$0.6$}}%
      \put(814,2526){\makebox(0,0)[r]{\strut{}$0.7$}}%
      \put(814,2786){\makebox(0,0)[r]{\strut{}$0.8$}}%
      \put(814,3047){\makebox(0,0)[r]{\strut{}$0.9$}}%
      \put(814,3307){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(946,484){\makebox(0,0){\strut{}$0.0$}}%
      \put(1685,484){\makebox(0,0){\strut{}$1.0$}}%
      \put(2425,484){\makebox(0,0){\strut{}$2.0$}}%
      \put(3164,484){\makebox(0,0){\strut{}$3.0$}}%
      \put(3904,484){\makebox(0,0){\strut{}$4.0$}}%
      \put(4643,484){\makebox(0,0){\strut{}$5.0$}}%
      \put(1316,3177){\makebox(0,0)[l]{\strut{}$\eta_{crtical}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(209,2005){\rotatebox{-270}{\makebox(0,0){\strut{}$\eta_\tau$}}}%
      \put(2794,154){\makebox(0,0){\strut{}$\taupp = Fo_p {Pr_p}^{1/3}$}}%
      \csname LTb\endcsname%%
      \put(3656,2335){\makebox(0,0)[r]{\strut{}$Pr_p = 57$}}%
      \csname LTb\endcsname%%
      \put(3656,2115){\makebox(0,0)[r]{\strut{}$\ \ \ \  14$}}%
      \csname LTb\endcsname%%
      \put(3656,1895){\makebox(0,0)[r]{\strut{}$\ \ \ \  8$}}%
      \csname LTb\endcsname%%
      \put(3656,1675){\makebox(0,0)[r]{\strut{}$\ \ \ \  6$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{Prp-4_values_at_Ref2Prf2Grp4}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figures/Ref-2_values_at_Prf1Prp1Grp1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(946,704){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(946,1390){\makebox(0,0)[r]{\strut{}$0.05$}}%
      \put(946,2076){\makebox(0,0)[r]{\strut{}$0.1$}}%
      \put(946,2762){\makebox(0,0)[r]{\strut{}$0.15$}}%
      \put(946,3447){\makebox(0,0)[r]{\strut{}$0.2$}}%
      \put(946,4133){\makebox(0,0)[r]{\strut{}$0.25$}}%
      \put(946,4819){\makebox(0,0)[r]{\strut{}$0.3$}}%
      \put(1078,484){\makebox(0,0){\strut{}$0.0$}}%
      \put(1896,484){\makebox(0,0){\strut{}$0.2$}}%
      \put(2714,484){\makebox(0,0){\strut{}$0.4$}}%
      \put(3532,484){\makebox(0,0){\strut{}$0.6$}}%
      \put(4349,484){\makebox(0,0){\strut{}$0.8$}}%
      \put(5167,484){\makebox(0,0){\strut{}$1.0$}}%
      \put(5985,484){\makebox(0,0){\strut{}$1.2$}}%
      \put(6803,484){\makebox(0,0){\strut{}$1.4$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(209,2761){\rotatebox{-270}{\makebox(0,0){\strut{}$\eta$}}}%
      \put(3940,154){\makebox(0,0){\strut{}$\tau = Gr_p \alpha t /D^2 $}}%
      \csname LTb\endcsname%%
      \put(5816,4646){\makebox(0,0)[r]{\strut{}$Re_f = 149$}}%
      \csname LTb\endcsname%%
      \put(5816,4426){\makebox(0,0)[r]{\strut{}$Re_f = 2090$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{Ref-2_values_at_Prf1Prp1Grp1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figures/Ref-2_values_at_Prf2Prp4Grp4.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(814,704){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(814,1116){\makebox(0,0)[r]{\strut{}$0.1$}}%
      \put(814,1527){\makebox(0,0)[r]{\strut{}$0.2$}}%
      \put(814,1939){\makebox(0,0)[r]{\strut{}$0.3$}}%
      \put(814,2350){\makebox(0,0)[r]{\strut{}$0.4$}}%
      \put(814,2762){\makebox(0,0)[r]{\strut{}$0.5$}}%
      \put(814,3173){\makebox(0,0)[r]{\strut{}$0.6$}}%
      \put(814,3585){\makebox(0,0)[r]{\strut{}$0.7$}}%
      \put(814,3996){\makebox(0,0)[r]{\strut{}$0.8$}}%
      \put(814,4408){\makebox(0,0)[r]{\strut{}$0.9$}}%
      \put(814,4819){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(946,484){\makebox(0,0){\strut{}$0.0$}}%
      \put(1783,484){\makebox(0,0){\strut{}$2.0$}}%
      \put(2619,484){\makebox(0,0){\strut{}$4.0$}}%
      \put(3456,484){\makebox(0,0){\strut{}$6.0$}}%
      \put(4293,484){\makebox(0,0){\strut{}$8.0$}}%
      \put(5130,484){\makebox(0,0){\strut{}$10.0$}}%
      \put(5966,484){\makebox(0,0){\strut{}$12.0$}}%
      \put(6803,484){\makebox(0,0){\strut{}$14.0$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(209,2761){\rotatebox{-270}{\makebox(0,0){\strut{}$\etafr$}}}%
      \put(3874,154){\makebox(0,0){\strut{}$\taufr = Gr_p \alpha t /D^2 $}}%
      \csname LTb\endcsname%%
      \put(5816,4646){\makebox(0,0)[r]{\strut{}$Re_f = 149$}}%
      \csname LTb\endcsname%%
      \put(5816,4426){\makebox(0,0)[r]{\strut{}$Re_f = 2090$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{Ref-2_values_at_Prf2Prp4Grp4}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figures/Ref-4_values_at_Prf1Prp1Grp2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5040.00,3528.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(814,704){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(814,964){\makebox(0,0)[r]{\strut{}$0.1$}}%
      \put(814,1225){\makebox(0,0)[r]{\strut{}$0.2$}}%
      \put(814,1485){\makebox(0,0)[r]{\strut{}$0.3$}}%
      \put(814,1745){\makebox(0,0)[r]{\strut{}$0.4$}}%
      \put(814,2006){\makebox(0,0)[r]{\strut{}$0.5$}}%
      \put(814,2266){\makebox(0,0)[r]{\strut{}$0.6$}}%
      \put(814,2526){\makebox(0,0)[r]{\strut{}$0.7$}}%
      \put(814,2786){\makebox(0,0)[r]{\strut{}$0.8$}}%
      \put(814,3047){\makebox(0,0)[r]{\strut{}$0.9$}}%
      \put(814,3307){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(946,484){\makebox(0,0){\strut{}$0.0$}}%
      \put(1474,484){\makebox(0,0){\strut{}$0.2$}}%
      \put(2002,484){\makebox(0,0){\strut{}$0.4$}}%
      \put(2530,484){\makebox(0,0){\strut{}$0.6$}}%
      \put(3059,484){\makebox(0,0){\strut{}$0.8$}}%
      \put(3587,484){\makebox(0,0){\strut{}$1.0$}}%
      \put(4115,484){\makebox(0,0){\strut{}$1.2$}}%
      \put(4643,484){\makebox(0,0){\strut{}$1.4$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(209,2005){\rotatebox{-270}{\makebox(0,0){\strut{}$\eta_\tau$}}}%
      \put(2794,154){\makebox(0,0){\strut{}$\taufr = Fo_p $}}%
      \csname LTb\endcsname%%
      \put(3656,1537){\makebox(0,0)[r]{\strut{}$Re_f = 149$}}%
      \csname LTb\endcsname%%
      \put(3656,1317){\makebox(0,0)[r]{\strut{}$\ \ \ \  796$}}%
      \csname LTb\endcsname%%
      \put(3656,1097){\makebox(0,0)[r]{\strut{}$\ \ \ \  1443$}}%
      \csname LTb\endcsname%%
      \put(3656,877){\makebox(0,0)[r]{\strut{}$\ \ \ \  2090$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{Ref-4_values_at_Prf1Prp1Grp2}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figures/Theta_Grp-4_values_at_Ref2Prf2Prp4.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(946,704){\makebox(0,0)[r]{\strut{}$10^{-6}$}}%
      \put(946,1292){\makebox(0,0)[r]{\strut{}$10^{-5}$}}%
      \put(946,1880){\makebox(0,0)[r]{\strut{}$10^{-4}$}}%
      \put(946,2468){\makebox(0,0)[r]{\strut{}$10^{-3}$}}%
      \put(946,3055){\makebox(0,0)[r]{\strut{}$10^{-2}$}}%
      \put(946,3643){\makebox(0,0)[r]{\strut{}$10^{-1}$}}%
      \put(946,4231){\makebox(0,0)[r]{\strut{}$10^{0}$}}%
      \put(946,4819){\makebox(0,0)[r]{\strut{}$10^{1}$}}%
      \put(1078,484){\makebox(0,0){\strut{}$0.0$}}%
      \put(2223,484){\makebox(0,0){\strut{}$1.0$}}%
      \put(3368,484){\makebox(0,0){\strut{}$2.0$}}%
      \put(4513,484){\makebox(0,0){\strut{}$3.0$}}%
      \put(5658,484){\makebox(0,0){\strut{}$4.0$}}%
      \put(6803,484){\makebox(0,0){\strut{}$5.0$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(209,2761){\rotatebox{-270}{\makebox(0,0){\strut{}$1 - \theta = 1 - \frac{T_{p}-T_{mean}}{T_{in}-T_{mean}}$}}}%
      \put(3940,154){\makebox(0,0){\strut{}$\taupg = Gr_p Fo_p (\times100000)$}}%
      \csname LTb\endcsname%%
      \put(5816,4646){\makebox(0,0)[r]{\strut{}$Gr_p = 24906$}}%
      \csname LTb\endcsname%%
      \put(5816,4426){\makebox(0,0)[r]{\strut{}$\ \ \ \  83021$}}%
      \csname LTb\endcsname%%
      \put(5816,4206){\makebox(0,0)[r]{\strut{}$\ \ \ \  141134$}}%
      \csname LTb\endcsname%%
      \put(5816,3986){\makebox(0,0)[r]{\strut{}$\ \ \ \  199248$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{Theta_Grp-4_values_at_Ref2Prf2Prp4}}%
    \gplfronttext
  \end{picture}%
\endgroup

